Spatiotemporal impacts of human activities and socio-demographics during the COVID-19 outbreak in the U.S

Understanding influencing factors is essential for the surveillance and prevention of infectious diseases, and the factors are likely to vary spatially and temporally as the disease progresses. Taking daily cases and deaths data during the coronavirus disease 2019 (COVID-19) outbreak in the U.S. as a case study, we develop a mobility-augmented geographically and temporally weighted regression (M-GTWR) model to quantify the spatiotemporal impacts of social-demographic factors and human activities on the COVID-19 dynamics. Different from the base GTWR model, we incorporate a mobility-adjusted distance weight matrix where travel mobility is used in addition to the spatial adjacency to capture the correlations among local observations. The model residuals suggest that the proposed model achieves a substantial improvement over other benchmark methods in addressing the spatiotemporal nonstationarity. Our results reveal that the impacts of social-demographic and human activity variables present significant spatiotemporal heterogeneity. In particular, a 1% increase in population density may lead to 0.63% and 0.71% more daily cases and deaths, and a 1% increase in the mean commuting time may result in 0.22% and 0.95% increases in daily cases and deaths. Although increased human activities will, in general, intensify the disease outbreak, we report that the effects of grocery and pharmacy-related activities are insignificant in areas with high population density. And activities at the workplace and public transit are found to either increase or decrease the number of cases and deaths, depending on particular locations. The results of our study establish a quantitative framework for identifying influencing factors during a disease outbreak, and the obtained insights may have significant implications in guiding the policy-making against infectious diseases.

==> liter.tex <==
\section{Literature Review}
The public authorities quickly responded to the infectious disease propagation through multiply strategies during the COVID-19 outbreak. For example, the government released the emergency statement, travel restrictions, city lockdowns, and social distance policy in the reopening plan. These actions aim to reduce human contacts in space and time, and real-world observations have proved the efficiency of these strategies. For example, the lockdown policies~\cite{brzezinski2020covid} in the U.S. increase the time that people spend at home to 39\%. Extensive travel restriction has been tested to reduce the cumulative attack rate by 77-87\% in the pandemic~\cite{degli2008mitigation}. Furthermore, existing studies have demonstrated the effects of social-demographic characteristics and mobility on disease propagation~\cite{mateus2014effectiveness}.


The social-demographic structure of the population has been proved to have significant effect on the fatality rate during the COVID-19 outbreak. The earliest study in China ~\cite{novel2020epidemiological} has shown that the order population with age greater than 80 years older have the highest fatality rate of 14.8\%. Later, studies~\cite{dowd2020demographic,sannigrahi2020overall} show the heterogeneous effect of the age structure is a global phenomenon. In addition, the study~\cite{almagro2020differential} in New York City has indicated the racial disparities persist among the Whites, Blacks, Asians, Hispanics in the COVID-19 outbreak. In particular, nearly 20\% of U.S. counties have a disproportionate Black population~\cite{millett2020assessing}, and they accounted for 52\% of COVID-19 diagnoses and 58\% of COVID-19 deaths nationally. Except for the effects of demographic structure, the social and economic criteria have also governed the extent of the COVID-19 disease propagation. The study~\cite{atchison2020perceptions} suggested the lowest household income were six times less likely to be able to work from home and three times less likely to be able to self-isolate in the U.K. during COVID-19. Besides, Viktor Stojkoski et al.,~\cite{stojkoski2020socio} mentioned the high-income population show higher resistance of being infected by the COVID-19.



The human motion provides the physical diffusion for the contagion propagation and is closely associated with the dynamical processes of the epidemiology evolution. Multiple studies have addressed the efficiency of human activities on contagion propagation. Studies~\cite{vazquez2013using, poletto2013human} suggested the geographic space significantly affects human mobility, then affects the epidemic propagation, and temporally irregular daily routines increase an epidemic’s final size. Bing Wang et al.,~\cite{wang2017interplay} suggested both information propagation and human mobility patterns co-affect the epidemic propagation. Nevertheless, Lima et al.,~\cite{lima2015disease} provided evidence that restricting mobility does not delay the occurrence of an endemic state. Bajardi et al.,~\cite{bajardi2011human} also addressed that stricter regimes of travel reduction would have led to delays in the order of two weeks, even in the optimistic case of early intervention based on the study in 2009 H1N1 pandemic.

The aforementioned studies have provided unprecedented insights for understanding the impact of social-demographic characteristics on the disease propagation. They assumed the effects to be fixed among time and space. However, the WHO study~\cite{mateus2014effectiveness} mentioned that the effect size and propagation efficiency vary among geographical sources, and the natural process of the disease propagation is spatial auto-correlated. Ignoring these effects leads to the loss of heterogeneity in the estimation. Besides, the existing studies reveal endogeneity issues due to the inter-dependency among the influencing factors, which results in biased estimates. In particular, the disease propagation efficiency varies cross contagions due to the magnitude of the infection rate and the recovery rate. Furthermore, although some studies have investigated the impacts of social-demographic characteristics on the COVID-19 propagation, most of them are based on the descriptive analysis. As a consequence, to address the aforementioned issues, a quantitative approach to examine the heterogeneous effects of COVID-19 remains to be explored. In this study, considering the spatial and temporal heterogeneity among counties in U.S. We investigated the effects of social-demographic characteristics, travel mode, and human activity on the COVID-19 propagation. The insights provide a valuable understanding of the effects of influencing factors on the COVID-19 propagation in U.S. metropolitan area. 

